Optimal Sensing Precision for Celestial Navigation Systems in Cislunar Space using LPV Framework

This paper introduces two innovative convex optimization formulations to simultaneously optimize the H2/Hinf observer gain and sensing precision, and guarantee a specified estimation error bound for nonlinear systems in LPV form. Applied to the design of an onboard celestial navigation system for cislunar operations, these formulations demonstrate the ability to maintain accurate spacecraft positioning with minimal measurements and theoretical performance guarantees by design.

==> lit_survey.tex <==
\section{Brief Review of LPV Systems}
%Linear Parameter Varying (LPV)\cite{shamma1990analysis, shamma2012overview} control systems represent an advanced approach in control theory for handling nonlinear systems by employing a family of linear controllers. These controllers are scheduled based on varying parameters that are measurable in real time. The LPV framework extends the gain scheduling approach, which traditionally involves designing controllers at various operating points and interpolating between them as system parameters change. The interpolated controller doesn't have theoretical guarantees. However, the LPV framework provides theoretical guarantees since the design accounts for parameter variations. Several methodologies exist for designing LPV controllers, including \textit{linear fractional transformations (LFT)}, \textit{single quadratic Lyapunov function (SQLF)}, and \textit{parameter dependent quadratic Lyapunov function (PDQLF)}. These methodologies reformulate control design problems into convex optimization problems involving linear matrix inequalities (LMIs) \cite{el2000advances,helton2007linear}. The main challenge is representing the nonlinear system as a linear parameter-varying system. For example, a nonlinear system $\dot{x} = x^3$ can be written as $\dot{x} =A(\rho)x$, where $A(\rho) = \rho$ with $\rho(t) := x^2(t)$. When LPV models are affine in the parameter, i.e., $A(\rho) = A_0 + A_1\rho$, the constraints to guarantee performance for all variation in $\rho(t)$ are simpler. It is assumed $\rho(t)$ is in a convex polytope, and guarantees are established with constraints defined on the vertices of the polytope. If the dependence on $\rho(t)$ is nonlinear, randomized algorithms are often employed with probabilistic guarantees \cite{tempo2013randomized, fujisaki2003probabilistic}.  Often, additional parameters are introduced to force an affine structure, resulting in many parameters. The computational burden increases with problem size and is dominated by the worst-case complexity of LMIs are $\mathcal{O}(n^6)$, where $n$ is the problem size. Also, restricting $\rho(t)$ in a closed set is often not trivial. Besides these limitations, the LPV framework has been quite successful, particularly in the aerospace industry \cite{ganguli2002reconfigurable, balas2002linear, gilbert2010polynomial, marcos2009lpv}. 

This \cite{9121301} addresses the problem of selecting a sparse set of sensors and determining the minimum required precision for observer design in linear time-invariant (LTI) systems. The authors propose an integrated theoretical framework that optimizes sensor precision and observer gain to achieve specified accuracy in state estimates, formulated within an $\mathcal{H}_2/\mathcal{H}_\infty$ optimal estimation framework. The optimization problem is posed as a convex problem, minimizing the l1 norm of the precision vector to achieve sparseness. The approach is applied to the linearized longitudinal model of an F-16 aircraft, demonstrating its effectiveness in designing \(\mathcal{H}_2/\mathcal{H}_\infty\) optimal observers with sparse sensor configurations while minimizing sensor precision. This work builds on existing literature by treating sensor precision as an unknown variable and directly scaling individual sensor channels to induce sparseness. The \cite{9121301} on maximizing sensor noise is going to be used as a primary reference in this paper as we implement its LMI with an LPV system and prove that using an LPV system does not change the LMI formulation. 

This \cite{MATTEI2004651} addresses the trajectory tracking control problem for propagation processes modeled as quasi-linear parameter varying systems. Typically described by partial differential equations (PDEs), these models are often converted into ordinary differential equations (ODEs) for practical control applications. The authors propose a trajectory following control scheme for systems with linear propagation dynamics and nonlinear boundary conditions. They also present a robust performance analysis based on quadratic stability with an \(\mathcal{H}_\infty\) norm bound and propose an LMI-based observer synthesis procedure to enhance closed-loop system performance. The article does not specifically address maximizing noise for controller performance

This paper \cite{PIGA2015329} reviews various methods for identifying LPV input-output models, highlighting the challenges posed by noise in both output and scheduling signal measurements. The authors propose a bias-corrected, instrumental-variable (IV) based method to address this issue, providing consistent estimates for LPV models with polynomial dependence on the scheduling variable. This method does not require an approximation of the noise-free scheduling signal, making it more practical for real-world applications. The paper also shows that neglecting noise on the scheduling signal can lead to significant bias in estimated parameters and presents an identification scheme to compute consistent estimates from noisy observations.

This \cite{zheng1998transfer} goes into two new bias-eliminated least-squares (BELS) algorithms are introduced for identifying linear systems with noisy input and output data. These algorithms estimate noise variances using a one-dimensional over-parameterization of the system transfer function. Simulation examples demonstrate their effectiveness. while this paper does not go into quantifying the affects of noise on controller performance it does go into some detail of how to get direct estimates of noisy data.

The \cite{9955878} proposes a fault detection (FD) method for discrete-time LPV systems with sensor faults and measurement noise. It introduces an interval FD observer using \(\mathcal{L}_\infty\) performance to minimize uncertainties and improve estimation accuracy. Additionally, \(\mathcal{L}_-\) performance is considered to calculate the sensitivity of the residual to sensor faults, setting a decision to indicate their presence. The methodology’s validity is demonstrated through a numerical example. The paper emphasizes the importance of designing fault detection observers that are robust against uncertainties and sensitive to faults, using performance indexes such as \(\mathcal{L}_\infty\), \(\mathcal{H}_\infty\), and \(\mathcal{L}_\infty\) norms.


This \cite{4663892} addresses the problem of selecting $k$ sensor measurements from $m$ potential options to minimize parameter estimation error. Evaluating all $(m, k)$ combinations is impractical for large $m$ and $k$. it proposes a heuristic based on convex optimization that provides an approximate solution and a performance bound. While the gap between the heuristic’s performance and the bound is not guaranteed to be small, numerical experiments show it often is.

The following sources set up fault tolerant systems. The \cite{s22176664} on virtual-sensor-based fault tolerant strategies explores strategies for fault tolerance using virtual sensors. The \cite{app8101816} on LPV model-based sensor fault diagnosis and isolation for permanent magnet synchronous generators in wind energy conversion systems focuses on sensor fault diagnosis and isolation using LPV models. Another \cite{9456971} delves into adaptive event-triggered finite-frequency fault detection with zonotopic threshold analysis for LPV systems. Lastly, the \cite{https://doi.org/10.1002/acs.1263} on robust fault detection based on adaptive threshold generation using interval LPV observers describes robust fault detection using adaptive threshold generation with interval LPV observers

It should be noted that quantifying maximum sensor degradation is not formulated and any of the LPV sources rather most relay on develop a series of fault tolerant systems. There for the novelty of this paper is derived from the utilizing the formulation in \cite{9121301} and show that for an affine LPV state space the formulation holds
